Considerations about the incompleteness of the Ehrenfest's theorem in quantum mechanics

We describe a study motivated by our interest to examine the incompleteness of the Ehrenfest's theorem in quantum mechanics and to resolve a doubt regarding whether or not the hermiticity of the hamiltonian operator is sufficient to justify a simplification of the expression of the macroscopic-observable time derivative that promotes the one usually found in quantum-mechanics textbooks. The study develops by considering the simple quantum system "particle in one-dimensional box". We propose theoretical arguments to support the incompleteness of the Ehrenfest's theorem in the formulation he gave, in agreement with similar findings already published by a few authors, and corroborate them with the numerical example of an electric charge in an electrostatic field. The contents of this study should be useful to Bachelor and Master students; the style of the discussions is tailored to stimulate, we hope, the student's ability for independent thinking.

==> popd-k=1-4.tex <==
\begin{figure}[h]
   \hspace*{\mathindent}
   \resizebox{\sfsize}{!}{\includegraphics*[trim=10 25 60 60]{\figdir/popd-k=1.eps}} 
   \resizebox{\sfsize}{!}{\includegraphics*[trim=10 25 60 60]{\figdir/popd-k=2.eps}} \\ 
   \hspace*{\mathindent}
   \resizebox{\sfsize}{!}{\includegraphics*[trim=10 25 60 60]{\figdir/popd-k=3.eps}} 
   \resizebox{\sfsize}{!}{\includegraphics*[trim=10 25 60 60]{\figdir/popd-k=4.eps}}     
   \caption{Position-operator probability density in the first four stationary states of an electric charge in uniform electrostatic field. \label{popd1-4.cef}}
\end{figure}

